On the Connection between Game-Theoretic Feature Attributions and Counterfactual Explanations

Explainable Artificial Intelligence (XAI) has received widespread interest in recent years, and two of the most popular types of explanations are feature attributions, and counterfactual explanations. These classes of approaches have been largely studied independently and the few attempts at reconciling them have been primarily empirical. This work establishes a clear theoretical connection between game-theoretic feature attributions, focusing on but not limited to SHAP, and counterfactuals explanations. After motivating operative changes to Shapley values based feature attributions and counterfactual explanations, we prove that, under conditions, they are in fact equivalent. We then extend the equivalency result to game-theoretic solution concepts beyond Shapley values. Moreover, through the analysis of the conditions of such equivalence, we shed light on the limitations of naively using counterfactual explanations to provide feature importances. Experiments on three datasets quantitatively show the difference in explanations at every stage of the connection between the two approaches and corroborate the theoretical findings.

==> assets/methods_equivalency_table.tex <==
%auto-ignore
\begin{tabular}{r|ccc}
\multicolumn{1}{r}{\textbf{}}                   & \textbf{Summary Technique}   & \textbf{Feature Removal}$^{*}$               & \textbf{Model Behaviour} \\
SHAP                                 & Shapley Values     & Training Set                                 & Prediction        \\
\textsc{Binary SHAP}                  & Shapley Values     & Training Set                                 & Binary Prediction        \\
CF-SHAP                            & Shapley Values     & Counterfactuals                              & Prediction        \\
\textsc{MaxSparse CF-SHAP}             & Shapley Values     & Maximally Sparse Counterfactuals             & Prediction        \\
\textsc{Binary CF-SHAP}                & Shapley Values     & Counterfactuals                              & Binary Prediction        \\
\textsc{Binary MaxSparse CF-SHAP}      & Shapley Values     & Maximally Sparse Counterfactuals             & Binary Prediction        \\

% \textbf{Binary MaxSparse Permutation Test}      & Remove Individual & Maximally Resilient Counterfactuals & Binary Prediction        \\
% \textbf{Binary MaxSparse CF-LIME}               & Linear Model       & Maximally Sparse Counterfactuals  & Binary Prediction        \\
% \itodo{???}                                    & Include Individual & Maximally Sparse Counterfactuals    & Binary Prediction        \\
% \itodo{\textbf{Binary MaxSparse RISE}}          & Mean When Included & \itodo{???}                         & Binary Prediction        \\
% \itodo{\textbf{Partitioned Subsets}}            & Partioned Subsets & \itodo{???}                         & Binary Prediction        \\
\end{tabular}
